Fast and Accurate Neural Word Segmentation for Chinese

Neural models with minimal feature engineering have achieved competitive performance against traditional methods for the task of Chinese word segmentation. However, both training and working procedures of the current neural models are computationally inefficient. This paper presents a greedy neural word segmenter with balanced word and character embedding inputs to alleviate the existing drawbacks. Our segmenter is truly end-to-end, capable of performing segmentation much faster and even more accurate than state-of-the-art neural models on Chinese benchmark datasets.

==> mpxerr.tex <==
\gdef\mpxshipout{\shipout\hbox\bgroup
  \setbox0=\hbox\bgroup}
\gdef\stopmpxshipout{\egroup  \dimen0=\ht0 \advance\dimen0\dp0
  \dimen1=\ht0 \dimen2=\dp0
  \setbox0=\hbox\bgroup
    \box0
    \ifnum\dimen0>0 \vrule width1sp height\dimen1 depth\dimen2 
    \else \vrule width1sp height1sp depth0sp\relax
    \fi\egroup
  \ht0=0pt \dp0=0pt \box0 \egroup}
\mpxshipout% line 17 ./fig.mp
$\mathbf{c}_1$%
\stopmpxshipout
\mpxshipout% line 18 ./fig.mp
$\mathbf{c}_L$%
\stopmpxshipout
\mpxshipout% line 19 ./fig.mp
$\mathbf{\hat{w}}$%
\stopmpxshipout
\mpxshipout% line 20 ./fig.mp
$\mathbf{w}$%
\stopmpxshipout
\mpxshipout% line 34 ./fig.mp
$\mathbf{r}_1 $%
\stopmpxshipout
\mpxshipout% line 35 ./fig.mp
$\mathbf{r}_L$%
\stopmpxshipout
\mpxshipout% line 36 ./fig.mp
$\mathbf{z}_N$%
\stopmpxshipout
\mpxshipout% line 37 ./fig.mp
$\mathbf{z}_1$%
\stopmpxshipout
\mpxshipout% line 38 ./fig.mp
$\mathbf{z}_L$%
\stopmpxshipout
\end{document}

